SoftNull: Many-Antenna Full-Duplex Wireless via Digital Beamforming

In this paper, we present and study a digital-controlled method, called SoftNull, to enable full-duplex in many-antenna systems. Unlike most designs that rely on analog cancelers to suppress self-interference, SoftNull relies on digital transmit beamforming to reduce self-interference. SoftNull does not attempt to perfectly null self-interference, but instead seeks to reduce self-interference sufficiently to prevent swamping the receiver's dynamic range. Residual self-interference is then cancelled digitally by the receiver. We evaluate the performance of SoftNull using measurements from a 72-element antenna array in both indoor and outdoor environments. We find that SoftNull can significantly outperform half-duplex for small cells operating in the many-antenna regime, where the number of antennas is many more than the number of users served simultaneously.

==> arrayPartitioning.tex <==
\section{Antenna Array Partition}\label{sec:partition}
In the previous section we presented the optimal precoder design of \softNull, for a given ($\numRx\times\numTx$) self-interference channel. 
We next empirically answer the second research question highlighted in the introduction: \emph{given the required number of transmit and receive antennas, what is the best way to partition the $M$ antennas into the transmit and receive sets.} Due to the combinatorial nature of the problem, the problem of finding the optimal antenna sets is NP-complete. For example, if $M=64$ and $\numTx = 32$, then there are ${64 \choose 32}\approx 1.8\times10^{18}$ possible combinations of transmit antenna sets. 

Since identifying the optimal partition is practically intractable, we focus on empirical insights using channel measurements collected using a many-antenna base station. We experimentally show that the heuristic of splitting the array into contiguous transmit and receive partitions along its smallest dimension leads to very good performance. In particular, our heuristic provides 25~dB \emph{better} suppression than the average suppression by a random partition. 

% \lin{Why this problem is important? Why this problem is hard? }. 
% \lin{Please always place the points/key findings upfront. Therefore, at the opening of this subsection, please summarize the key insights}

%\lin{Some materials from other sections may be consolidated into below. We may want to create structure for this section as well by using subsections}
\subsection{Heuristic Partitions}

\begin{figure*}[ht]
\renewcommand{\subcapsize}{\normalsize}
\centering
	\subfigure[East-West\label{fig:EastWestSplit}]{
	\centering
	\input{DocGraphics/36x36LeftRightSplit.tex}	
	}
	\subfigure[North-South \label{fig:NorthSouthSplit}]{
	\centering
	\input{DocGraphics/36x36NorthSouth.tex}
    	}
	\subfigure[Northwest-Southeast (NW-SE) \label{fig:DiagSplit}]{
	\centering
	\input{DocGraphics/36x36NW-SE.tex}
	}
	\subfigure[Interleaved \label{fig:Interleaved}]{
	\centering
	\input{DocGraphics/36x36InterLeaved.tex}
	}
\caption{Tx/Rx selection heuristics: blue is transmit, red is receive. %\evanNote{I will adjust the geometry so it reflects the hexagonal pattern of the array we used}
}
\label{fig:partitions}
\end{figure*}


%\evanNote{Will add some text here setting up the problem and explaining why it is analytically intractable.}

%We saw in the example of Section~\ref{sec:example} that the array geometry -- the spatial relationship between transit and receive antennas -- greatly affects how well \softNull\ can suppress self-interference for a given number of transmit degrees-of-freedom sacrificed. 
%Therefore we would like to thoroughly explore the space of transmit and receive antennas selections for a fixed array -- that is, given an array of $\numTotal$ antennas and a requirement that $\numTx$ antennas be used for transmission and  $\numRx$ be used for reception, which antennas should we choose for reception and which for transmission? Unfortunately, this antenna selection problem is a NP-hard problem, however we propose and evaluate a heuristic approach to the antenna selection problem. 

%We know that \softNull\ will perform the best when the self-interference channel is approximately low rank, that is when the power in the in the self-interference channel is is concentrated within a fewer number of eigen channels. Less precisely, we want self-interference channels that are ``poorly conditioned.'' In physical wireless channels, the angular spread of the angles of arrival and angles of departure are what dictate how well or poorly a channel is conditioned. If the angular spread is large the channel is well conditioned, else the channel is poorly conditioned. Therefore one heuristic is to minimize the angular spread of the transmit array relative to the receive array. Minimizing the angular spread


\begin{figure*}[htb]
\renewcommand{\subcapsize}{\normalsize}
\centering
	\subfigure[36 Tx, 36 Rx\label{fig:36tx36rx-HeuristicCompare}]{
	\centering
	\input{DocPlots/compareAntennaSelectionsChamber.tex}	
	}
	\subfigure[48 Tx, 24 Rx]{
	\centering
	\input{DocPlots/compareAntennaSelectionsChamber48tx24rx}
    	}
\caption{Achieved \tradeoff\ for different Tx/Rx partitions of $9\times8$ rectangular array.}
\label{fig:partitionsResults}
\end{figure*}

%\begin{figure}[htb]
%\renewcommand{\subcapsize}{\normalsize}
%\centering
%	\centering
%	%\subfigure[36 Tx, 36 Rx\label{fig:36tx36rx-HeuristicCompare}]
%	\input{DocPlots/compareAntennaSelectionsChamber.tex}	
%\caption{Achieved \tradeoff\ for different Tx/Rx partitions of $9\times8$ rectangular array, with $(\numTx,\numRx) = (36,36)$. We note that the general trend is similar 
%%\evanNote{I could add plots like this for any pairing of $(\numTx,\numRx)$, such as asymmetric cases. But results is same in terms of the performance ordering. In previous draft I had a (48,24) split, but felt it wasn't adding much.}
%}
%\label{fig:partitionsResults}
%\end{figure}



Intuitively, we recognize that \softNull\ will perform the best when the power in the self-interference channel is concentrated within a fewer number of eigenchannels.   %. In physical wireless channels, the well-conditioned-ness of a channel is related to the angular spread between the transmitter and receiver. 
It been demonstrated both analytically and experimentally \evanNote{cite} that as the the spread of and angles-of-departure to/from transmitter to the receiver is decreased, the received at each receive antenna become more correlated, and hence the first few eigenvalues become more dominant, which is exactly the desirable situation for \softNull. Contiguous linear partitions of the array (one side transmit, other receive) limit the angular spread of the angles-of-departure to/from transmitter to the receiver by ensuring that all the interference is at least coming from only one ``side'' of the array (for example in the North-South partition of Figure~\ref{fig:NorthSouthSplit} the the angular spread of angles-of-arrival is less than 180 degrees of all receive antennas, since all interference is coming from the ``North''). 

Figure~\ref{fig:partitions} shows three proposed partitions based on the above heuristic of linear contiguous partitioning to limit angular spread: East-West, North-South, and Northwest-Southwest partitions are shown in Figures~\ref{fig:EastWestSplit},~\ref{fig:NorthSouthSplit}, and \ref{fig:DiagSplit} in the portion of the array is used, and equal numbers are transmit and receive. 

As a comparison, we also will consider the interleaved partition shown in Figure~\ref{fig:Interleaved}. If our heuristic of minimizing angular spread is a good one, then we would expect the interleaved partition to be a near worst-case partition - as in this configuration receive antennas see interference arriving at every possible angle. 
In addition to the deterministic interleaved partition, we will also compare against the average measured performance of $10,000$ randomly chosen partitions.

%The overall self-interference power will also be effected simply by the proximity of the transmit antennas and receive antennas: with transmit and receive antennas being right  totally separate heuristic one could employ is

%Therefore we proposed portioning the array into contiguous sets of transmit and receive antennas, one side is all transmit and one side is all receive (as opposed to an interlocking pattern of transmit and receive antennas). 

\subsection{Heuristic Evaluations}

\begin{figure}[t]
\centering
	\centering
	\includegraphics[width = 0.3\textwidth, clip=true, trim = 0 0 0 30cm]{DocGraphics/ArrayFromFront.jpg}
\caption{Planar antenna array used for self-interference channel measurements. \ashuNote{NASA is visible}}
\label{fig:arrayPic}
\end{figure}
To assess the performance of these heuristics, we directly measured the self-interference channel response in an anechoic chamber using the 72-element rectangular array shown in Figure~\ref{fig:arrayPic}. See the appendix for further detail on the measurement setup. 
Figure~\ref{fig:partitionsResults} shows the the \tradeoff\ achieved by \softNull, as measured in an anechoic chamber, for each of the three heuristic contiguous partitions, the interleaved partition, and the average of $10,000$ random partitions. 

%We have a noise floor of $-95$~dBm and transmit power of $0$~dBm, which limits the best achievable cumulative suppression  $-95+10\log(36) \approx -80$~dB.  

First note that all three linear contiguous partitions perform much better than than random partitions. For the random partition, we can only maintain $6$ of the maximum $36$ transmit dimensions while achieving  $>50$~dB suppression, but for all of the heuristic partitions,  we can achieve $>50$~dB suppression with at least 16 transmit dimensions preserved. 

Second, the best performing partition is the East-West partition, which is in line with our heuristic: among the four partitions, the East-West partition is the one with minimum angular spread between the transmit and receive partitions, since it splits the array along its smallest dimension (array is wider than tall). The interleaved partition performs even worse than the average of random partitions, emphasizing the importance of selecting contiguous partitions. 

Lastly, note the enormous impact of the partition selection, for downlink degrees-of-freedom between 3 and 22, the the East-West enables \softNull~to achieve more than $25$~dB more suppression than the average randomly chosen partition. We note the characterization of the relative performance of the partitions is performed in the anechoic chamber to ensure we are only affected by the array geometry, and not the local scattering. In practice local scattering will impact the optimal partition; however due to the NP-hardness of finding the optimal, we fix the form of partition to East-West for the rest of the performance evaluation.


==> motivation.tex <==
% !TEX root = main.tex

We next define the multi-user system under consideration and provide necessary background in multiuser MIMO and full-duplex wireless to motivate our solution, \softNull. 


\subsection{System Defintion}

We consider the multi-user cell system pictured in Figure~\ref{fig:problem}. A base station is communicating with $\numUplink$ uplink users and $\numDownlink$ downlink users\footnote{We assume the set of users were chosen by a scheduler, and hence their choice is not part of the current problem formulation.}. 
%\ashuNote{We need to clarify that all antennas can transmit and receive, like in a usual system. But none are full-duplex by themselves, we use some for transmit and others for receive. This can be flexibly done (again a scheduler's choice).} 
The base station is equipped with $\numTotal$ antennas. We assume the base station uses traditional radios, that is each of the $M$ antennas can both transmit and receive, but a given antenna cannot both transmit and receive at the same time (at the same frequency). 
 A subset $\numTx$ of the $\numTotal$ antennas are used for downlink transmission and $\numRx$ antennas for uplink reception. Since each antenna is connected to a standard radio which can switch between transit and receive modes, but does not both transmit and receive simultaneously. Therefore in full-duplex operation, $\numTx$ of the antennas transmit while $\numRx$ antennas receive, with the requirement that $\numTx + \numRx \leq \numTotal$. Note that choice of which antennas transmit and receive is flexible and adaptable (for example, can be chosen by a scheduler). In half duplex mode all antennas are used for either transmission or reception, that is $\numTx = \numRx = \numTotal$.  The vector of symbols transmit by the base station is $\bsTx \in \mathbb{C}^{\numTx}$, and the vector of symbols transmitted by the users is $\usrTx \in \mathbb{C}^{\numUplink}$. Of course the elements of   $\bsTx$ can be jointly designed by the base station, whereas each user can only control its own corresponding element of $\usrTx$. 

The signal received at the base station is 
\begin{equation}
\label{eq:uplinkChannel}
\bsRx = \upChannel \usrTx +  \selfChannel  \bsTx  + \bsNoise,
\end{equation}
where $\upChannel \in \mathbb{C}^{\numRx\times\numUplink}$  is the uplink channel matrix, $\selfChannel \in \mathbb{C}^{ \numRx \times \numTx}$ is the self-interference channel matrix, $\bsNoise \in \mathbb{C}^{\numRx}$ is the receiver noise. The signal received by the $\numDownlink$ downlink users is
\begin{equation}
\label{eq:downlinkChannel}
\usrRx = \downChannel \bsTx  + \interuserChannel \usrTx +  \usrNoise,
\end{equation}
where $\downChannel \in \mathbb{C}^{\numDownlink \times \numTx}$,  is the downlink channel matrix, $\interuserChannel \in \mathbb{C}^{\numDownlink \times \numUplink}$ is the matrix of channel coefficients from the uplink to the downlink users,  and $\usrNoise \in \mathbb{C}^{\numDownlink}$ is the noise at each user's receiver.  

In this work we focus only on the challenge of self-interference.  Research on the  scheduling problem of selecting uplink and downlink users who have very weak inter-user interference channels for full-duplex transmission is actively ongoing \cite{Tang15ADuplex, Kim13Janus, Singh2011FDMAC, Gai14FDScheduling, Suhas15FDScheduling} (and references therein). Thus, unless otherwise stated, we will generally assume $\interuserChannel = 0$. In half-duplex operation the above equations are simplified: the self-interference term is eliminated in (\ref{eq:uplinkChannel}), and $\upChannel$ is a $\numTotal \times \numUplink$ matrix and $\numDownlink$ is a  $\numDownlink \times \numTotal$ matrix. The signaling challenges in this topology are 1) how to design $\bsTx$ so that each downlink user receives only the signal intended for that user (i.e. precoding), 2) how to process $\bsRx$ to separate the signals from each user (i.e. equalization) and 3) how to design $\bsTx$ such that the self-interference is small. Challenges 1) and 2) have been well studied and are reviewed below, Challenge 3), which is obviously coupled with Challenge 1), is the focus of this paper, and is discussed in its own section, Section~\ref{sec:precoder}. 

\begin{figure}[ht]
\centering
%\includegraphics[width=0.5\textwidth]{DocGraphics/types-of-interference.pdf} 
\input{DocGraphics/sytemFigure.tex}
\caption{Multi-user full-duplex system \evanNote{Figure in progress}
\label{fig:problem}}
\end{figure}



\subsection{Multiuser MIMO Background}

%Figure~\ref{fig:mumimo} depicts a multiple-user (MU) multiple-input multiple-output (MIMO) wireless communication system.

\ashuNote{For our journal audience, we most likely do not need this section. This was good for MobiCom community. Write the paper as journal paper, assuming sophisticated PHY audience.}
Multiple antennas can be used to support multiple data streams simultaneously to multiple users, with techniques generally known as Multiuser MIMO (MU-MIMO). 
The optimal (that is, capacity achieving) downlink signaling strategy is  Dirty Paper Coding \cite{}, but Dirty Paper Coding is often considered too computationally expensive for practical deployments \cite{}.
However, two suboptimal  signaling strategies for downlink MU-MIMO, studied widely in the literature, are zero-forcing beamforming (ZFBF) and matched filtering (MF). In ZFBF, the base-station precodes each user's data with the objective to deliver maximal energy to the user's receiver while nulling interference to other users. While ZFBF requires joint optimization of the precoders for all the users, matched filtering uses the precoder that is optimal for a user assuming there are no other users in the system. Multiple users can also be supported on uplink via receive beamforming (often also called equalization), where the receiver combines the received signal with different weights, to isolate different users' data. Conceptually, transmit and receive beamforming  are duals of each other, and zero-forcing beamforming and matched filtering have the analogous meaning for uplink equalization as for downlink precoding. 





\ashuNote{This is awkward way of referring to concepts - "so-called" - feels like you do not like them. And no reason for quotes. Also this para is too long.}
The so-called ``massive'' MIMO regime, in which the number of transmit/receive antennas is much more than the number of users being served, has gained much attention in recent years \cite{DBLP:journals/corr/abs-1304-6690}. 
Leveraging very large antenna arrays has many advantages, but there are two main advantages that stand out. The first advantage of very large arrays is that  simple suboptimal precoding techniques such as zero-forcing beamforming  and matched filtering perform nearly as well as the optimal Dirty Paper Coding in the large-array limit. The second advantage is that intercell-interference is suppressed in the large-array limit without requiring base station coordination. 
In the large array limit the spatial footprint of the signal to each user becomes highly focused in a small area around each user, meaning that interference to any other uses is suppressed, regardless of whether the base station has knowledge of that user.  Thus interference to users both registered with that base station and registered with other base stations is suppressed. 


% could enable as much as twice the physical layer data rate, and also provide the higher network layers many advantages that come with co-channel simultaneous transmission (lower latency, \evanNote{Maybe Lin add something}). 

\subsection{Full-Duplex and MIMO Self-Interference Cancellation Background}


\ashuNote{Remove this section. We will use the main concepts in introduction. Section 2 is only problem definition/formulation, like our other journal papers.}
Traditionally the MU-MIMO uplink and downlink are operated either on alternating time slots (time division duplex), or on separate frequency bands (frequency division duplex). Enabling MU-MIMO full-duplex at the infrastructure opens up many new modes for scheduling, by increasing the set of available physical layer modes. That is, depending on the channel conditions and network demand, the best choice may be to  have only uplink or downlink traffic in specific time-slots, and full-duplex operation in other time-slots. Furthermore,  full-duplex MU-MIMO infrastructure can support half-duplex mobiles and does not require mobile nodes to implement full-duplex. The last point is important since mobile data traffic need not be bi-directional~\cite{Falaki:2010:FLT:1879141.1879176}.
%\ashuNote{argh, need to say that mobile traffic is not all bi-directional, a good citation on mobile traffic will be useful}  


MIMO full-duplex presents many engineering challenges. All existing full-duplex, single or multiple antenna, require the use of additional analog circuits to enable cancellation of self-interference. Analog cancellation is essential since self-interference can be much more powerful than the received uplink signal, the self-interference will desensitize the receive electronics. Thus, to enable full-duplex, the self-interference must be suppressed \emph{prior} to the receiver analog-to-digital conversion; in fact, preferably before down-conversion.

The best known implementations of MIMO analog cancellation scale analog complexity linearly with the number of antennas~\cite{Katti2014FullDuplexMIMO}, where a general M-antenna design was proposed and experimentally evaluated only for a $3\times 3$ MIMO link. The linear complexity growth, while best possible, is challenging to implement and scale. The design in~\cite{Katti2014FullDuplexMIMO} requires tunable multi-tap analog filters, that require programmable analog delay and gain elements. It is well known that analog filters are not desirable in practice since their implementation does not benefit from Moore's laws, are expensive and power-hungry. Thus, implementing $O(M)$ multi-tap analog filters will be undesirable in practical systems for very large number of antennas, like 64-antenna system being considered in 3GPP. A nulling based design was proposed in~\cite{Aryafar12MIDU}, which requires careful placement of many antennas to create nulls at the receiving antennas. In this case, low analog complexity is traded with high antenna complexity; the design requires $4M$ antennas for a $M$-antenna MIMO system. The authors only evaluated the design for a $3\times 3$ MIMO link. 

An alternate design for MIMO full-duplex was presented in~\cite{Duarte2012FullDuplexWiFi} that only uses passive analog adders. Again, the authors only evaluated their design for 2$\times 2$ MIMO link. While the overall analog circuit requirements are much simpler compared to~\cite{Katti2014FullDuplexMIMO}, the cancellation design is fundamentally limited by the transmitter phase noise~\cite{Sahai13PhaseNoise}. In~\cite{yin2013full}, the authors proposed a zero-forcing precoder to create nulls at all receiving antennas. However, no experiments were performed. As discussed in the introduction and supported by our data in Section~\ref{sec:eval}, nulling based approaches leave very few or no degrees of freedom for actual downlink transmissions. 

We note that all of the above papers aimed to build a full-duplex $M\times M$ link, and not a full-duplex multiuser MIMO. In addition, the past designs were experimentally validated only for small antenna configurations (no more than $M=3$ antennas).%\lin{the above said 3 by 3 MIMO. That's 3 antennas, right? Should no more than 3, right?}.


%The overarching challenge is suppressing self-interference: each for the $\numTx$ transmit antennas will be dumping high-powered interference into the $\numRx$. Because this 

%Existing full-duplex wireless systems employ additional analog components for self-interference, including XYZ, XYZ, XYZ \lin{Fill in the names of the components}. These analog components not only are expensive but also incur additional design and implementation complexity.  The cost and complexity grow almost proportionally to the number of base station antennas, as shown in Table~\ref{tab:analog_cost}.\lin{Ashu mentioned you had a table showing how the number of analog components needed as related to the number of antennas. Please bring it back.}. More importantly, recent theoretical analysis and experimental results have shown that phase noise inherent to these analog components can considerably reduce the effectiveness of analog cancellation\lin{cite Ashu's paper, quantify the reduction, refine this sentence}, casting doubt on their practical performance.


%\lin{I merged the rest of the section, challenges and insights, into the intro. They were commented off below}

\begin{comment}
\subsection{Challenges toward All-Digital Full-Duplex Wireless}


Given the growing cost and complexity of the additional analog components employed by existing full-duplex systems and their questionable practical performance, we contribute an all-digital architecture, called \emph{SoftNull}, that suppress self-interference prior to the receiver only via digital design of the transmit signal, on top of existing radio hardware.

SoftNull employs nulling, a traditional approach in array beamforming for digital design to remove interference. In terms of matrix theory if we think about the channel between the transmit and receive antennas as a matrix of complex numbers (amplitudes and phases), then nulling is equivalent to projecting the transmit signal onto the nullspace of the channel. If channels are full-rank, then the rank nullity theorem dictates that each null created corresponds to a transmit degree-of-freedom sacrificed -- each null created is like sacrificing a transmit antenna. 


\subsubsection{Challenge 1: Optimal Precoder Design}


\subsubsection{Challenge 2: Full-duplex performance}


\subsubsection{Challenge 3: Antenna array partition}


\begin{figure}[htb]
\renewcommand{\subcapsize}{\normalsize}
\centering
\includegraphics[width = 0.3\textwidth, clip=true, trim=0 0 0 30cm]{DocGraphics/ArrayFromFront.jpg}
\caption{72-element patch antenna array}
\label{fig:array}
\end{figure}


\begin{figure}[htbp]
\begin{center}
%\input{DocGraphics/channelsAreFullRank.tex}
\includegraphics[width=0.5\textwidth]{DocGraphics/conditionHist.eps}
\caption{Histogram of condition number for measured self-interference channels: demonstrates channels are full rank. \evanNote{Maybe a better way of illustrating this concept is just showing that the nullspace is empty for nearly all channels...}}
\label{fig:channelRanks}
\end{center}
\end{figure}






\subsection{Old materials}
\lin{I don't quite understand the rest of the materials. So I leave them below.} 


\lin{first sentence should be the point of the paragraph. What's the point of this paragraph?} Conventional wireless wisdom states that MIMO channels are full rank and well conditioned in multi-path environments, but are rank deficient (or at least poorly conditioned) in open space (or line-of-sight-dominated environments). This convention breaks down, however, when the transmit array and receive array are in proximity, as in the case of a self-interference channel. Each receive antennas sees a ``different view'' of the the transmit array, meaning that each receive antenna will receive an independent linear combination of the signals from the transmit antennas: leading to full-rank and well conditioned channels. 

To assess this hypothesis that self-interference channels will not be low-rank, we took a 72-element path antennas array, shown in Figure~\ref{fig:array} into a large anechoic chamber, which mimics the conditions of open space, and measured the self-interference channel for many different partitions of transmit and receive antennas: left-right, top-bottom, diagonal-diagonal and 1,000 other randomly chosen partitions)\lin{this is a terrible sentence. Not only is it long but also it does not tell the point: Did you show the hypothesis to be true or false? }. Figure~\ref{fig:channelRanks} shows the histogram of the condition number of the self-interference channels. Factoring in noise, we expect a condition number of more than 90~dB for a rank deficient channel. Note that very few of the measured channel are even close to being rank defficient. This means that \emph{nulling self-interference is a zero-sum game}: every receive antenna one nulls is taking away an effective transmit antennas, cutting the downlink performance in proportion to the boost in uplink performance. 

\begin{figure}[htbp]
\begin{center}
\input{DocGraphics/eigenvaluesConcentrated.tex}
\caption{Distribution of eigenvalues for $(\numTx,\numRx) = (36,36)$ top-bottom transmit/receive antenna partition: power concentrated in dominant eigenchannels.}
\label{fig:eigenvalues}
\end{center}
\end{figure}


However, our measurements also demonstrate an opportunity. Figure~\ref{fig:eigenvalues} plots the distribution of eigenvalues for a $(\numTx,\numRx) = (36,36)$ top-bottom transmit/receive antenna partition.  Although the the channels are full rank, the self-interference power is concentrated in the first few eigenvalues of the channel. For example, $85\%$ of the power in the channel lies in the the first $10$ eigenchannels. Recall the whole that reason that receiver-side digital cancellation alone is insufficient is that the self-interference swamps the receiver analog electronics. However, Figure~\ref{fig:eigenvalues} suggests that there is an opportunity to suppress self-interference to a manageable level by avoiding the dominant eigenchannels, and allowing digital cancellation to do the rest. 
Our precoder, \softNull\, exploits this concentration of power to suppress the self-interference without sacrificing near the transmit degrees of freedom that would have been needed for explicit nulling. 

\input{otherChallenges}

\end{comment}

